On solving basic equations over the semiring of functional digraphs

Endowing the set of functional graphs (FGs) with the sum (disjoint union of graphs) and product (standard direct product on graphs) operations induces on FGs a structure of a commutative semiring R. The operations on R can be naturally extended to the set of univariate polynomials R[X] over R. This paper provides a polynomial time algorithm for deciding if equations of the type AX=B have solutions when A is just a single cycle and B a set of cycles of identical size. We also prove a similar complexity result for some variants of the previous equation.

==> tikzlibraryoodgraph.code.tex <==
%
% OODGraph: One Out-Degree Graphs library
%
% This library draws connected graphs with out-degree one. To draw unconnected OOD graphs, just draw separatedly their connected components
%
%\RequirePackage{etoolbox}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% This code below have been borrowed from etoolbox package  ----|          %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %%V% % % %
\newcommand*{\oodgraph@csxdef}[2]{\expandafter\xdef\csname#1\endcsname{#2}}
\newcommand*{\oodgraph@ifcsdef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
\newcommand*{\oodgraph@ifcsundef}[1]{%
  \ifcsname#1\endcsname
    \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\expandafter
      \expandafter\@firstoftwo
    \else
      \expandafter\expandafter
      \expandafter\@secondoftwo
    \fi
  \else
    \expandafter\@firstoftwo
  \fi}
\newcommand*{\oodgraph@csuse}[1]{%
  \ifcsname#1\endcsname
    \csname#1\expandafter\endcsname
  \fi}
\newcommand{\oodgraph@cslet}[2]{%
    \expandafter\let\csname#1\endcsname#2}
\newcommand*{\oodgraph@csgundef}[1]{\global\oodgraph@cslet{#1}\relax}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % A %
% The above code have been borrowed from etoolbox package  ----| %
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%
% Version 0.1 (2019/05/25):
% - first public release
% Version 0.2 (2019/06/01):
% - added /.store in key
% - added /.default key
% - cleaned up code
% Version 0.3 (2019/06/14)
% - fixed drawing algorithm
% - points definitions are now saved in a list
% - the points list is emptied at the closing of the environment oodgraph
% Version 0.4 (2019/06/18)
% - now commands are completely scoped
% - redisigned the graph printing algorithm to take into account that now
%    everything is scoped
% Version 0.45 (2019/06/19)
% - added the option 'rotation angle'
% Version 0.46 (2019/06/20)
% - added the option 'node content'
% - added bridge to tikz and pgf when a key is not known
% - made the library independent of 'etoolbox' package (borrow
%    some code from the package)
% - added oodgraph@ prefix to all commands so to avoid conflicts with other
%    packages/libraries
% Version 0.47 (2019/06/28)
% - options 'oodgraph arrow' and 'oodgraph node' renamed into 'oodgraph edges' and 'oodgraph nodes' for more consistancy
% - fixed a bug with edges style
% - now '->' is the default edge style
% Version 0.48 (2019/07/14)
% - added a check in \addorigin to verifiy if the point has been defined before
% - some code polishing (eliminated the list oodgraph@more@options which is no
%    more used, deleted \oodgraph@resetkeys function and integrated its code
%    directly into the calling functions since its body contained only an \end{scope}
%    command, deleted several unuseful \expandafter commands)
% - explicited the definition of oodgraph@csxdef
% - partially rewritten the drawing routine for beards. Now it is much faster
% Version 0.50 (2019/07/15)
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - renamed style options 'oodgraph nodes' into 'nodes style' which is shorter and nicer
% - introduced the option 'loop style' which allows to style the loops
% - fixed a bug for the special case of cycles of order 2 which drawn the two edges
%   one over the other (obtening a double arrow). Thanks to François Doré for signalling
%   this.
% - bug fix: the beards to be wrongly oriented when the xshift key
%   was used in the addcycle command. Bug discovery and fix by François Doré
% - bug fix: when a cycle had only 2 nodes, they addresses where exchanged. Thanks
%   to François Doré for signalling this
% Version 0.51 (2024/04/24)
% - added the option 'rotation angle' for \addcycle
% - added the option 'loop angle' for \addcycle therefore removing in and out option from the base loop style
% - added the option 'attach margin' for \addbeard to make edges stop further away from the beard tip in order to prevent them from intertwining when there are many of them
% - bug fix: when a cycle had only 1 node, the default angle of the beard does not match the shape of the loop
% - bug fix: the 'opening angle' option was wrongly computed
% - merged addbeard cases with 1 or 1+ nodes
% - changed the bend option in the case of a cycle of two nodes to preserve counter-clockwise order for every case
% - changed to polar coordinates for some of the node positioning
% - changed base node shapes to circles


\def\fileversion{0.51}
\def\filedate{2024/04/24}
\message{Library OODGraph}
\message{ v.\ \fileversion, \filedate}
% load tikz dependencies
\usetikzlibrary{calc}
\makeatletter
\gdef\oodgraph@tmp{}
\gdef\oodgraph@points@list{}
%
% convenience routines to extract the prefix from a node path
%
\def\oodgraph@get@prefix@from@path@@#1-#2\pgf@eov{\xdef\oodgraph@tmp{\oodgraph@csuse{#1.origin}}}
\def\oodgraph@get@prefix@from@path#1{
\pgfutil@in@{-}{#1}
\ifpgfutil@in@% if there is a minus sign then it is a package defined point
\oodgraph@get@prefix@from@path@@#1\pgf@eov
\else% regular pgf/tikz point
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\xdef\oodgraph@tmp{(\XCoord,\YCoord)}
\fi
}
%
%  oodgraph@addtolist
%  #1 = name of the list to add to
%  #2 = object to be added
% Service function to append objects to lists
%
\newcommand*{\oodgraph@addtolist}[2]{%
   \expandafter\if\expandafter\relax\csname #1\endcsname\relax%
      \expandafter\expandafter\xdef\csname #1\endcsname{#2}%
   \else%
    \expandafter\xdef\csname #1\endcsname{\csname #1\endcsname,#2}%
\fi%
}
%
%  oodgraph@docslist@undeft
%  #1 = separator char
%  #2 = name of the list
% Service routine to \csundef all elements of the list
% 
\newcommand{\oodgraph@docslist@undef}[2][,]{%
%   #1 = separation char
%   #2 = list
   \def\dolist##1{\expandafter\@dolist##1#1\@eol}%
   \def\@dolist##1#1##2\@eol{%
   % process stuff here with ##1
   \oodgraph@csgundef{##1}
   \ifx\@eol##2\@eol\else\@dolist##2\@eol\fi}%
   \dolist{#2}%
}
%
\pgfkeys{/oodgraph/.search also={/tikz, /pgf}} %,/oodgraph/catch unknown}}%
%\pgfkeys{/oodgraph/.search also={/tikz,/pgf,/oodgraph/catch unknown}}%
\pgfkeys{%
/oodgraph/.cd,
%radius/.initial={1},
radius/.value required,
radius/.default={1},
radius/.store in=\oodgraph@radius,
radius,
%attach node/.initial={a->1},
attach node/.value required,
attach node/.default={a->1},
attach node/.store in=\oodgraph@attach@node,
attach node,
%nodes prefix/.initial={a},
nodes prefix/.value required,
nodes prefix/.default={a},
nodes prefix/.store in=\oodgraph@nodes@prefix,
nodes prefix,
%opening angle/.initial={120},
opening angle/.value required,
opening angle/.default={60},
opening angle/.store in=\oodgraph@opa,
opening angle,
rotation angle/.value required,
rotation angle/.default={0},
rotation angle/.store in=\oodgraph@rota,
rotation angle,
attach margin/.value required,
attach margin/.default={},
attach margin/.store in=\oodgraph@attach@margin,
attach margin,
loop angle/.value required,
loop angle/.default={100},
loop angle/.store in=\oodgraph@loop@angle,
loop angle,
nodes content/.value required,
nodes content/.default={$\bullet$},
nodes content/.store in=\oodgraph@node@content,
nodes content,
nodes@style/.style={circle,inner sep=1pt},
edges@style/.style={->},
loop@style/.style={looseness=6},
nodes style/.code=\pgfkeys{/oodgraph/nodes@style/.style={#1}},
edges style/.code=\pgfkeys{/oodgraph/edges@style/.style={#1}},
loop style/.code=\pgfkeys{/oodgraph/loop@style/.style={#1}},
semi thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={semi thick}},
thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={thick}},
ultra thick/.code=\pgfkeys{/oodgraph/edges@style/.append style={ultra thick}},
edges color/.code=\pgfkeys{/oodgraph/edges@style/.append style={#1}},
nodes color/.code=\pgfkeys{/oodgraph/nodes@style/.append style={#1}},
}
%\pgfkeys{/oodgraph/.unknown/.code={%
%\ifx#1\pgfutil@empty\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname}\else\oodgraph@addtolist{oodgraph@more@options}{\pgfkeyscurrentname=#1}
%\fi}}
%
\newenvironment{oodgraph}[1][]{\begin{scope}[#1]}
{% closing the environment
% free all points definition in the current list
%\forcsvlist{\csgundef}{\oodgraph@points@list}
\expandafter\oodgraph@docslist@undef\expandafter{\oodgraph@points@list}
% free the points list
\gdef\oodgraph@points@list{}
% free temporary definitions
\gdef\oodgraph@tmp{}
\end{scope}}
%
\newcommand{\oodgraph@processkeys}[1][]{
\begin{scope}
\pgfkeys{/oodgraph/.cd,#1}
}
\long\def\oodgraph@drawcycle#1;{
\ifnum#1=1\oodgraph@drawcycle@\else%
{\ifnum#1=2\oodgraph@drawcycle@@{#1}\else%
\oodgraph@drawcycle@@@{#1}\fi}\fi%
% record circle center on points list and define it
\path(0,0);\pgfgetlastxy{\XCoord}{\YCoord};%
\oodgraph@ifcsundef{\oodgraph@nodes@prefix.origin}{%
% if undefined then add to the point list
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}%
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix.origin}%
}%
{% if already defined then simply replace the old definition
\oodgraph@csxdef{\oodgraph@nodes@prefix.origin}{(\XCoord,\YCoord)}%
}%
\end{scope}
}
%
\newcommand{\oodgraph@drawcycle@}{
%\pgfcoordinate{myorigin}{\pgfpointorigin}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at (\oodgraph@rota:.02){\oodgraph@node@content};
% save point on the list
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
%\expandafter\oodgraph@csxdef\expandafter{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(0pt,0pt)}
% draw edge
\pgfmathsetmacro{\inloopvalue}{180-\oodgraph@loop@angle/2+\oodgraph@rota}
\pgfmathsetmacro{\outloopvalue}{180+\oodgraph@loop@angle/2+\oodgraph@rota}
\draw[/oodgraph/edges@style]
(\oodgraph@nodes@prefix->1) edge[/oodgraph/loop@style,in=\inloopvalue,out=\outloopvalue] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@}{
% second node
\pgfmathsetmacro{\oodgraph@half@radius}{.5*\oodgraph@radius}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->2) at (\oodgraph@rota:-\oodgraph@half@radius){\oodgraph@node@content};
% first node
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->1) at (\oodgraph@rota:\oodgraph@half@radius){\oodgraph@node@content};
% register nodes
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->1}
\oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->2}
\oodgraph@csxdef{\oodgraph@nodes@prefix->1}{(-\oodgraph@half@radius,0pt)}
\oodgraph@csxdef{\oodgraph@nodes@prefix->2}{(\oodgraph@half@radius,0pt)}
% draw edges
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->1) edge[/oodgraph/edges@style, bend right] (\oodgraph@nodes@prefix->2);
\draw[/oodgraph/edges@style] 
(\oodgraph@nodes@prefix->2) edge[/oodgraph/edges@style, bend right] (\oodgraph@nodes@prefix->1);
}
\newcommand{\oodgraph@drawcycle@@@}[1]{
\pgfmathsetmacro\stepangle{360.0/#1}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\nodeangle{(\i-1)*\stepangle+\oodgraph@rota}
\node[/oodgraph/nodes@style](\oodgraph@nodes@prefix->\i) at (\nodeangle:\oodgraph@radius){\oodgraph@node@content};
  \path(\oodgraph@nodes@prefix->\i); \pgfgetlastxy{\XCoord}{\YCoord};
  \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@nodes@prefix->\i}
  \oodgraph@csxdef{\oodgraph@nodes@prefix->\i}{(\XCoord,\YCoord)}
}
%\wlog{list=\oodgraph@points@list}
\foreach \i in {1,...,#1}{
  \pgfmathsetmacro\nodeimage{ifthenelse(\i==#1,int(1),int(\i+1))}
  \draw[/oodgraph/edges@style] (\oodgraph@nodes@prefix->\i) -- (\oodgraph@nodes@prefix->\nodeimage);
}
}
\newcommand*{\addcycle}[1][]{%
\oodgraph@processkeys[#1]%
\oodgraph@drawcycle%
}
%
\def\addorigin#1;{%
\pgfutil@ifundefined{pgf@sh@ns@#1}{
\edef\mymsgtmp{No point named #1\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the point has been correctly defined via the standard TikZ interface.}
}{%
\path(#1);\pgfgetlastxy{\XCoord}{\YCoord};
\oodgraph@csxdef{#1}{(\XCoord,\YCoord)}%
\oodgraph@csxdef{#1.origin}{(\XCoord,\YCoord)}%
%\oodgraph@addtolist{oodgraph@points@list}{#1} % added v. 0.48
%\oodgraph@addtolist{oodgraph@points@list}{#1.origin} % added v. 0.48
}}
%
\newcommand{\addbeard}[1][]{%
\oodgraph@processkeys[#1]
\oodgraph@drawbeardlev
}
\def\oodgraph@drawbeardlev#1;{%
%\wlog{list=\oodgraph@points@list}
\oodgraph@drawbeardlev@@{#1}
\end{scope}}
\newcommand{\oodgraph@drawbeardlev@@}[1]{
% #1= number of nodes in the level
% check if the attachment node has been previously defined
\oodgraph@ifcsdef{\oodgraph@attach@node}{% then part
% if the attach node has been defined then
% find the root prefix and retrive the origin
\expandafter\oodgraph@get@prefix@from@path\expandafter{\oodgraph@attach@node}
\path[reset cm]\oodgraph@tmp;\pgfgetlastxy{\XOCoord}{\YOCoord};
\path[reset cm](\oodgraph@attach@node);\pgfgetlastxy{\XCoord}{\YCoord};
}% end of then part
{% if it is not defined, print an error message
\edef\mymsgtmp{No point named \oodgrap@attach@node\space has been found!}
\PackageError{OODGraph}\mymsgtmp
{Please verify that the attachment node has been correctly defined or that there exists a addorigin command.}
}%
\begin{scope}[shift={(\XOCoord, \YOCoord)}]
% recompute coordinates of attach point in the new coordinate system
\pgfmathsetmacro\XCoord{\XCoord-\XOCoord}
\pgfmathsetmacro\YCoord{\YCoord-\YOCoord}
% compute angle wrt attachment point
\pgfmathsetmacro\originangletmp{atan(\YCoord/(\XCoord+.01))}
\pgfmathsetmacro\originangle{ifthenelse(\XCoord>=0,\originangletmp,180+\originangletmp)}
% compute lowest angle
\pgfmathsetmacro\startangle{\originangle+\oodgraph@rota+(\oodgraph@opa/2)*ifthenelse(#1==1,0,1)}
% compute angle between two nodes
\pgfmathsetmacro\stepangle{\oodgraph@opa/ifthenelse(#1==1,1,#1-1)}

\foreach \i in {#1,...,1}{
\pgfmathsetmacro\curangle{\startangle-(#1-\i)*\stepangle}

\node[/oodgraph/nodes@style](\oodgraph@attach@node->\i) at ($(\oodgraph@attach@node)+(\curangle:\oodgraph@radius)$){\oodgraph@node@content};
\ifx\oodgraph@attach@margin\empty%
{\draw[/oodgraph/edges@style] (\oodgraph@attach@node->\i) -- (\oodgraph@attach@node);}\else%
{\draw[/oodgraph/edges@style] (\oodgraph@attach@node->\i) -- ($(\oodgraph@attach@node->\i)!\oodgraph@attach@margin!(\oodgraph@attach@node)$);}\fi%

  % save points to points@list
  \path(\oodgraph@attach@node->\i); \pgfgetlastxy{\XCoord}{\YCoord};
 \oodgraph@addtolist{oodgraph@points@list}{\oodgraph@attach@node->\i}
 \oodgraph@csxdef{\oodgraph@attach@node->\i}{(\XCoord,\YCoord)}
}
\end{scope}
}
%
\makeatother
%
\endinput
